Understanding Longitudinal Behaviors of Toxic Accounts on Reddit

Toxic comments are the top form of hate and harassment experienced online. While many studies have investigated the types of toxic comments posted online, the effects that such content has on people, and the impact of potential defenses, no study has captured the long-term behaviors of the accounts that post toxic comments or how toxic comments are operationalized. In this paper, we present a longitudinal measurement study of 929K accounts that post toxic comments on Reddit over an 18~month period. Combined, these accounts posted over 14 million toxic comments that encompass insults, identity attacks, threats of violence, and sexual harassment. We explore the impact that these accounts have on Reddit, the targeting strategies that abusive accounts adopt, and the distinct patterns that distinguish classes of abusive accounts. Our analysis forms the foundation for new time-based and graph-based features that can improve automated detection of toxic behavior online and informs the nuanced interventions needed to address each class of abusive account.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> conversational.tex <==
%\subsection{Conversational Toxicity}
%% Where on the platform does this toxicity happen? In response to a post? In
%% response to a comment? Provide these distributions, and talk about how it's
%% really 50/50, and sometimes accounts are triggered by nothing, they just want
%% to be toxic. One thing this section can benefit from is example quotes where
%% an account is just being aggressive from the get go.
%
%% We can do the dyad labeling like Saveski did, with tox, not_tox, talk about
%% the likelhood that toxicity follows a reply, however, maybe it doesn't that
%% much because its' 50/50.
%
%% What to say about conversation trees? We can talk about their depth, we can
%% talk about how what happens when a toxic interaction happens in the tree, and
%% discuss how that matches up with other things. Like, do toxic interactions
%% escalate the conversation?
%
%\dk{How do abusive accounts engage with targets of abuse on the
%platform? In reply to a post? In reply to a comment? How do these interactions
%compare to abusive interactions on other platforms?}
%
%Abusive accounts in our study post toxic content on Reddit in two ways: they can
%either comment directly on a post (i.e., start a new comment tree) or reply to
%another comment that is already posted (i.e., reply). To study these
%interactions, we reconstructed 4.3M~comment trees that contained toxic
%interactions with abusive accounts during our observation period. Of these, Of
%these, 2.4M (55.5\%) are started by an abusive account and are a direct reply
%to a post. The remaining 1.9M (45.5\%) are nested reply trees, where an
%abusive account posts a toxic comment in reply to another comment.
%
%Prior research has studied the conversational structure of toxic interactions on
%other platforms, such as Twitter~\cite{saveski2021structure} and
%Wikipedia~\cite{conversationsawry}. To better understand toxic conversations on
%Reddit, we study toxicity at both a \emph{dyad} level and a conversation-tree
%level.
%
%\paragraph{Dyads.}
%\todo{Big problem in this section is that it assumes a blanket level of
%toxicity---perhaps we only look at abuser account interactions and call it a
%day.}
%\dk{How frequently is toxic behavior triggered by a toxic comment? When a toxic
%comment is posted, how frequently is it met with toxicity?}
%
%A dyad denotes a comment pair, which in this case is either a toxic reply to a
%comment or a reply left to a toxic comment on the platform. We tag each dyad by
%whether the originating comment and responding comment is toxic or not toxic,
%using a threshold of \texttt{SEVERE\_TOXICITY} $>$ 0.7. We also note whether
%each comment was created by an abusive account or a nonabusive account.
%
%70\% of the original comments that were met with toxic behaviors were \emph{not}
%toxic, highlighting that abusive accounts may tend to escalate the toxicity of


==> dead.tex <==
%\paragraph{Comparison to prior research with varying thresholds.}
%Prior research has used various Perspective API thresholds to maximize for
%precision. All rely on relatively small samples for threshold selection. For
%example, Hua et~al.\, chose a Perspective threshold of 0.7 based on a manually
%labeled sample of 100~tweets~\cite{hua2020towards}.

Because we only compare interactions with subreddits in isolation, we are
comfortable relaxing our Perspective API threshold when comparing user behavior
to the subcommunities they participate in.

In this context, we relax our Perspective API constraint as we are using it as a
relative measure rather than an absolute one.

We note that relaxing our Perspective API constraint will inherently
trigger more false positives, however, our norm metric is a \emph{relative}
measure and not an absolute one.

In our work, we add additional context to these existing defenses by highlighting which defenses may be most effective for varied types of abusive accounts. 

Other work has broadly focused on how 

Zhang et~al.\, observed that certain early warning signs can signal the eventual
collapse of civil conversation~\cite{conversationsawry, zhang2020quantifying},
while Chang et~al.\, highlight specifically how analyzing conversation flow with
context can aid in forecasting personal attacks~\cite{changtrouble}.
Furthermore, our work is directly related to prior work that suggests that
typically non-offending users can exhibit antisocial or abusive behavior if
given the right context~\cite{cheng2017anyone}, which is a precursor to our
hypotheses around ``one-off'' abuser behavior.


Finally, a chief goal of our work is to understand how our results can inform new time-based and graph-based features that can aid in defenses against toxicity. 


\paragraph{Community norms.}
We rely on a number of studies focused specifically on Reddit to inform our
experimental design and analysis choices. Prior work has investigated moderation
and toxicity norms on Reddit~\cite{rajadesingan2020quick,
chandrasekharan2018internet} and identified that subreddits exhibit unique
macro, meso, or micro-norms for moderation, highlighting challenges in
applying a broad definition of toxicity throughout the entire platform. To
control for these social phenomena in our work, we specifically look at abusive
behavior as \emph{derivations} from the established toxicity norms of a
community. Beyond norms, other studies investigated cross community movement and
shifts in toxicity following notable bans~\cite{chandrasekharan2017you,
chandrasekharan2019crossmod, ribeiro2020does}.

\paragraph{Attackers and targets.}
Recent studies have focused on the adversarial nature of toxic content
content and studied accounts that post toxic content online. Most similar to
our work, Ribeiro et~al.\ studied abuser properties on Twitter with the aim of
detecting hateful users based on their previous comments and their place in the
social graph~\cite{ribeiro2018characterizing}. Their work primarily focuses on
properties of accounts, for example, identifying follower-following ratios and
account age as a signal for hateful behavior. Past work has also focused on the
targets of abuse, observing that users are often targeted due to their race,
behaviors, and physical attributes~\cite{silva2016analyzing}. Beyond abusive
behavior in aggregate, several studies have looked at case studies of abuse. For
example, Hua et~al.\, identify specific properties of abusers that adversarially
interact with political candidates on Twitter~\cite{hua2020towards,
hua2020characterizing}. Prior work has also investigated a number of fringe hate
groups and online communities, including discourse on
Gab~\cite{zannettou2018gab}, Dissenter~\cite{rye2020reading}, the
Manosphere~\cite{horta2020evolution}, and 4chan's politically incorrect
board~\cite{papasavva2020raiders}. Instead of focusing on account properties,
our work instead contributes a longitudinal analysis of abuser \emph{behaviors}
across their entire account history, which can motivate nuanced defenses.

\paragraph{Online abuse and spam.}
Within the security community, our work is most closely aligned with the recent
body of work in online hate and harassment~\cite{thomas2021hate}, which
represents a shifting landscape of online abuse from for-profit cybercrime.
Toxic content bears the closest resemblance to spam, in that it is often
unwanted content with harmful consequences to platform users. As such, our work
borrows from prior work in measuring and mitigating
spam~\cite{grier2010spam,levchenko2011click} that focuses on account behaviors,
and prior work that studies graph-based spam
propagation~\cite{nilizadeh2017poised}.

% Conversational
\paragraph{Early warnings of toxic behavior.}
Finally, our work draws on computational studies of online conversation. Zhang
et~al.\, observed that certain early warning signs can signal the eventual
collapse of civil conversation~\cite{conversationsawry, zhang2020quantifying},
while Chang et~al.\, highlight specifically how analyzing conversation flow with
context can aid in forecasting personal attacks~\cite{changtrouble}.
Furthermore, our work is directly related to prior work that suggests that
typically non-offending users can exhibit antisocial or abusive behavior if
given the right context~\cite{cheng2017anyone}, which is a precursor to our
hypotheses around ``one-off'' abuser behavior.


%, particularly as existing classifiers (e.g., those on Facebook) flag just 5\% of %toxic content on the platform~\cite{wp-facebook-detection}.

%\indent Toxic comments are the top form of hate and harassment experienced
%online~\cite{thomas2021hate}. Transparency reports from Meta estimate that
%0.14--0.15\% of all views on Facebook in 2021 were of toxic
%posts~\cite{facebook-transparency-toxic}; Twitter reports that it removed
%roughly two million accounts in the second half of 2020 due to hate and
%harassment~\cite{twitter-transparency-toxic}. Experiencing these attacks can
%lead users to self-censor to avoid further attacks or outright leave online
%%platforms~\cite{powers2019shouting,thomas2022s}. In many cases, such attacks
%also serve as the entry point for more sophisticated security attacks, like
%a%ccount compromise, doxxing, and
%cyberstalking~\cite{leslie-jones,leslie-jones-hack,aliapoulios2021large,eileen%-huang}.

%Many online hate and harassment attacks draw closest parallels to classic
%for-profit cybercrime. Toxic content, for example, is closest to online spam,
%and receiving a barrage of toxic comments all at once is similar to for-profit
%distributed denial-of-service (DDoS). Given these similarities, the security
%community is well poised to build on existing anti-abuse research help curb %toxic
%content online~\cite{thomas2021hate}. Techniques used in prior work, like
%studying spam propagation through underlying graph
%structures~\cite{nilizadeh2017poised} and leveraging temporal perspectives in
%sybil defenses~\cite{liu2015exploiting} proved useful in tackling classic %abuse.
%Similar measurements of toxic content can inform the types of defenses---such %as %nudges, warnings, and bans---that might best reduce online harassment.

Historically, protections in social media have focused on fraudulent accounts that strictly engage in automated posting~\cite{thomas2013trafficking}; or compromised accounts that briefly post
abusive content from an otherwise benign account until the legitimate owner
regains control~\cite{egele2013compa}. Our findings indicate that users who post
toxic comments represent an entire new class of abusive account. The majority of
these accounts engage in abusive infractions throughout their lifetime, but
simultaneously contribute significant volumes of non-toxic content, ostensibly
making them valuable contributors to the platform at large. As such, traditional
strategies for dealing with abusive accounts (\eg mass account bans) are likely
untenable, as they would significantly reduce meaningful conversation on the
platform and have potentially unforeseen consequences on platform health. Some
platforms are attempting more nuanced actions. For example, Twitter deployed a
strike system for handling accounts that post Covid-19
misinformation~\cite{twitter-strike}, and some subreddits have implemented
similar strike systems for moderation at large~\cite{programmer-strike}. Still,
there is limited insight into how effective these strategies may be for handling
online hate and harassment. The design of new defensive schemes and evaluating
their efficacy for these types of attacks is a promising area of future
research.


==> related.tex <==
\section{Related Work}

Our work leverages insights and techniques from several other empirical studies
of toxic behavior online:

\paragraph{Attackers and targets.} Most similar to our work, Ribeiro et~al.\
studied abuser properties on Twitter with the aim of detecting hateful users
based on their previous comments and their place in the social
graph~\cite{ribeiro2018characterizing}. Their work primarily focuses on
properties of accounts, for example, identifying follower-following ratios and
account age as a signal for hateful behavior. Past work has also focused on the
targets of abuse, observing that users are often targeted due to their race,
behaviors, and physical attributes~\cite{silva2016analyzing}. Beyond abusive
behavior in aggregate, several studies have looked at case studies of abuse. For
example, Hua et~al.\, identify specific properties of abusers that adversarially
interact with political candidates on Twitter~\cite{hua2020towards,
hua2020characterizing}. Prior work has also investigated a number of fringe hate
groups and online communities, including discourse on
Gab~\cite{zannettou2018gab}, Dissenter~\cite{rye2020reading}, the
Manosphere~\cite{horta2020evolution}, and 4chan's politically incorrect
board~\cite{papasavva2020raiders}. Instead of focusing on account properties,
our work instead contributes a longitudinal analysis of abuser \emph{behaviors}
across their entire account history, which can motivate nuanced defenses.

%\kt{Consider adding 1 sentence that differentiates our work from these?}

\paragraph{Community norms.}
We rely on a number of studies focused specifically on Reddit to inform our
experimental design and analysis choices. Prior work has investigated moderation
and toxicity norms on Reddit~\cite{rajadesingan2020quick,
chandrasekharan2018internet} and identified that subreddits exhibit unique
macro-, meso-, or micro-norms for moderation, highlighting challenges in
applying a broad definition of toxicity throughout the entire website. To
control for these social phenomena in our work, we specifically look at abusive
behavior as \emph{derivations} from the established toxicity norms of a
community. Beyond norms, other studies investigated cross community movement and
shifts in toxicity following notable bans~\cite{chandrasekharan2017you,
chandrasekharan2019crossmod, ribeiro2020does}.

% Conversational
\paragraph{Early warnings of toxic behavior.}
Our work draws on computational studies of online conversation. Zhang
et~al.\, observed that certain early warning signs can signal the eventual
collapse of civil conversation~\cite{conversationsawry, zhang2020quantifying},
while Chang et~al.\, highlight specifically how analyzing conversation flow with
context can aid in forecasting personal attacks~\cite{changtrouble}.
Furthermore, our work is directly related to prior work that suggests that
typically non-offending users can exhibit antisocial or abusive behavior if
given the right context~\cite{cheng2017anyone}, which is a precursor to our
hypotheses around ``one-off'' abuser behavior.

